GeAR: Graph-enhanced Agent for Retrieval-augmented Generation

Retrieval-augmented Generation (RAG) relies on effective retrieval capabilities, yet traditional sparse and dense retrievers inherently struggle with multi-hop retrieval scenarios. In this paper, we introduce GeAR, a system that advances RAG performance through two key innovations: (i) an efficient graph expansion mechanism that augments any conventional base retriever, such as BM25, and (ii) an agent framework that incorporates the resulting graph-based retrieval into a multi-step retrieval framework. Our evaluation demonstrates GeAR's superior retrieval capabilities across three multi-hop question answering datasets. Notably, our system achieves state-of-the-art results with improvements exceeding 10% on the challenging MuSiQue dataset, while consuming fewer tokens and requiring fewer iterations than existing multi-step retrieval systems. The project page is available at https://gear-rag.github.io.

==> Appendices/correlation_between_hops_and_agent_iters.tex <==
\section{Correlation between Question Hops and Agent Iterations}
\label{appendix_sec:correlation_between_hops_and_agent_iterations}

\begin{figure*}[tbhp]
  \includegraphics[width=\textwidth]{figures/experiments/hop_vs_agent_iteration_correlation.pdf}
  \caption{Analysis of the relationship between the number of hops in questions and the required number of agent iterations for the MuSiQue dataset. For each hop count, we analyse the number of iterations required by \gear to determine question answerability. The maximum iteration limit was set to 4, with ``4+'' indicating cases where the agent could not determine answerability within this limit. The visualization presents two complementary perspectives on the same data: the left panel shows a box plot emphasizing the median and distribution of stopping iterations, while the right panel focuses on the mean number of iterations across different hop counts.}
  \label{fig:hop_vs_agent_iteration_correlation}
\end{figure*}

The left panel in Figure \ref{fig:hop_vs_agent_iteration_correlation} demonstrates that the median stopping iteration remains consistently at 1 across all hop counts. Additionally, the upper quartile shows a clear upward trend as the number of hops increases. This suggests greater variability in processing time for more complex questions. The right panel illustrates two concurrent trends: as the question hop count increases, the number of questions in the dataset decreases, and the mean number of iterations \gear requires to determine question answerability increases. This pattern indicates that higher-hop questions not only appear less frequently but also typically demand more computational effort to process.

